In-processing User Constrained Dominant Sets for User-Oriented Fairness in Recommender Systems

Recommender systems are typically biased toward a small group of users, leading to severe unfairness in recommendation performance, i.e., User-Oriented Fairness (UOF) issue. The existing research on UOF is limited and fails to deal with the root cause of the UOF issue: the learning process between advantaged and disadvantaged users is unfair. To tackle this issue, we propose an In-processing User Constrained Dominant Sets (In-UCDS) framework, which is a general framework that can be applied to any backbone recommendation model to achieve user-oriented fairness. We split In-UCDS into two stages, i.e., the UCDS modeling stage and the in-processing training stage. In the UCDS modeling stage, for each disadvantaged user, we extract a constrained dominant set (a user cluster) containing some advantaged users that are similar to it. In the in-processing training stage, we move the representations of disadvantaged users closer to their corresponding cluster by calculating a fairness loss. By combining the fairness loss with the original backbone model loss, we address the UOF issue and maintain the overall recommendation performance simultaneously. Comprehensive experiments on three real-world datasets demonstrate that In-UCDS outperforms the state-of-the-art methods, leading to a fairer model with better overall recommendation performance.

==> chapters/the_proposed_framework/dominant_set_and_constrained_dominant_set.tex <==
\subsection{Technical Preparation for \M}
\nosection{Dominant Sets}
%
Given a graph $G=(\mathcal{V}, \mathcal{E}, w)$, where $\mathcal{V} = \{v1, v2, \dots, v_z\}$ indicates the vertex set with $z$ represents the number of vertices, $\mathcal{E} \in \mathcal{V} \times \mathcal{V}$ indicates the edge set, and $w:E \xrightarrow{} R_+^*$ is the positive weight function.
%
The weight of an edge reflects the similarities between the linked vertices.
%
We represent the graph $G$ with an weighted adjacency matrix $\mathbf{H} \in R^{| \mathcal{V} | \times | \mathcal{V} |}$, which is non-negative and symmetric.
%
$\mathbf{H}_{ij}$ is defined as $w(i, j)$ if $(i, j) \in \mathcal{E}$, and $0$ otherwise.
%
Note that there are no self-loops in $G$, thus all entries on the main diagonal of $H$ is zero.

%
Dominant sets generalizes the concept of a maximal clique to construct clusters in an edge-weighted graph.
%
As introduced and proved in \cite{pavan2006dominant}, we can extract a node cluster by solving the following linear-constrained quadratic optimization problem:
%
\begin{equation}
\label{dominant-sets-equ}
    \begin{split}  
    &\text{maximize} \ f(x) = x^{'} \mathbf{H}x,
    \\ 
    &\text{subject to} \ x \in \bigtriangleup, 
    \end{split}
\end{equation}
%
where $\bigtriangleup$ is the standard simplex of $R^z$:
\begin{equation}
\label{triangle-equ}
    \bigtriangleup = \{x \in R^z: \sum_{i = 1}^{z} x_i = 1, \text{and} \ x_i \ge 0 \ \text{for all} \ i = 1, 2, \dots, z\}.
\end{equation}

%
According to $x$, we can extract how relevant a node is to the cluster.
%
A effective way to solve the optimization above is the so-called \textit{replicator dynamics}, which is defined as follows:
\begin{equation}
    \label{replicator-dynamic-equ}
    x_i^{t+1} = x_i^{t} \frac{(\mathbf{H}x^t)_i}{(x^t)^{'}\mathbf{H}x^t}.
\end{equation}

\nosection{Constrained Dominant Sets}
%
Constrained dominant sets is an extension to dominant sets.
%
The key idea is that by choosing one or more nodes as constraints, we can extract a cluster containing such user-selected elements.
%
The constrained dominant sets can also be defined as a optimization problem as follows:
%
\begin{equation}
    \label{constrained-dominant-set-equ}
    \begin{split}
        &\text{maximize} \ f_\mathcal{S}^\alpha(x) = x^{'} (\mathbf{H} - \alpha \hat{\mathbf{I
}}_\mathcal{S})x,
        \\ 
        &\text{subject to} \ x \in \bigtriangleup, 
    \end{split}
\end{equation}
%
where $\mathcal{S}$ indicates the user-selected elements set, $\hat{\mathbf{I
}}_\mathcal{S}$ is the $z \times z$ diagonal matrix whose element is set to $1$ in correspondence to the vertices contained in $\mathcal{V} \backslash \mathcal{S}$ and $0$ otherwise.
%
Note that if $\alpha = 0$, the above optimization problem will degenerate to dominant sets.
%
Similar to Equation \ref{dominant-sets-equ}, the optimization problem \ref{constrained-dominant-set-equ} can also be solved as follows:
%
\begin{equation}
    \label{constrainted-replicator-dynamic-equ}
    x_i^{t+1} = x_i^{t} \frac{((\mathbf{H} - \alpha \hat{\mathbf{I
}}_\mathcal{S})x^t)_i}{(x^t)^{'}(\mathbf{H} - \alpha \hat{\mathbf{I
}}_\mathcal{S})x^t}.
\end{equation}

==> chapters/the_proposed_framework/overview.tex <==
\subsection{Overview}
%
In this paper, we propose a novel in-processing \textbf{U}ser \textbf{C}onstrained \textbf{D}ominant \textbf{S}ets framework, namely UCDS, to better solve the user-oriented fairness issue in the recommendation task.
%
As shown in Figure \ref{overall-framework}, the overall framework is divided into two parts, i.e., the \textit{UCDS modeling process} (shown in blue) and the \textit{in-processing training process} (shown in green).
%
(1) UCDS can be seen as a complementary model for the backbone recommendation model.
%
Before the training process begins, we first extract a constrained cluster for each disadvantaged user.
%
Note that the advantaged users in each cluster are similar users to the target disadvantaged user identified by constraint dominant sets.
%
(2) During the training process, we calculate the embedding difference between each disadvantaged user and users in its cluster and generate the fairness loss.
%
We combine the fairness loss with the backbone recommendation model loss to simultaneously solve the fairness issue and enhance the overall recommendation performance.

%
In the following sections, we will first give the technical preparation for \M.
%
Then we will introduce the detail of the \M~modeling process and the in-processing training process.


==> chapters/the_proposed_framework/problem_formulation.tex <==
\subsection{Preliminary}

\nosection{Problem Formulation}
%
We use $\mathcal{U}$ and $\mathcal{I}$ to represent the user set and the item set, respectively.
%
We divide users into disadvantaged user group $\mathcal{T} = \{T_1, T_2, \dots, T_{M-1}, T_M\}$ and advantaged user group $\mathcal{A} = \{A_1, A_2, \dots, A_{N-1}, A_N\}$ based on their activity levels, where M and N indicate the number of users in each group.
%
According to \cite{li2021user, rahmani2022experiments}, various behaviors (i.e., interactions, total consumption, and max trade price) can all reflect users' activity levels.
%
Since recommendation models are always trained directly based on user-item interactions, without loss of generality, we choose users' interaction numbers (users with more interactions are more likely to be advantaged) to group users.
%
In this paper, we aim to narrow the gap in the recommendation performance between $\mathcal{T}$ and $\mathcal{A}$ to achieve user-oriented fairness and improve the overall recommendation performance simultaneously.
%
% Besides, we also want to enhance the overall recommendation performance of the backbone model by solving the fairness issue.

User-oriented fairness is a kind of group fairness \cite{hardt2016equality, dwork2012fairness}.
%
The principle of group fairness is to ensure groups of users with different protected sensitive attributes should be comparably treated.
%
According to this idea, the definition of user-oriented fairness is defined as follows \cite{li2021user, rahmani2022experiments}:
%
\begin{definition}[User-Oriented Fairness (UOF)]
\begin{equation}
\label{user-oriented-fairness}
    \mathbb{E}[\mathcal{M(\mathcal{A})}] = \mathbb{E}[\mathcal{M(\mathcal{T})}],
\end{equation}
\end{definition}
%
where $\mathcal{M}$ indicates a metric (i.e. NDCG, F1-score) that can evaluate the recommendation performance. We use $\mathcal{M}(u)$ to represent the recommendation performance of user $u$.

%
UOF aims to offer users with different activity levels the same recommendation performance, which is usually impossible in real-world RS.
%
Thus researchers \cite{li2021user, rahmani2022experiments} always calculate the difference in average recommendation performance for different user groups to evaluate the fairness of a model:

\begin{definition}[The UOF matric (\UOFMatric)]
\begin{equation}
\label{user-oriented-fairness-cal}
    \mathcal{M}_{UOF}(\mathcal{T}, \mathcal{A}) = \bigg | \frac{1}{\lvert \mathcal{A} \rvert} \sum_{A_i \in \mathcal{A}} \mathcal{M}(A_i) - \frac{1}{\lvert \mathcal{T} \rvert} \sum_{T_i \in \mathcal{T}} \mathcal{M}(T_i) \bigg |.
\end{equation}
\end{definition}

%
In this paper, we use the value of \UOFMatric~to evaluate the fairness of a recommendation model. 
%
A smaller \UOFMatric~means a fairer algorithm that tends to treat different activity groups of users equally.

\nosection{Technical Preparation for \M}
%


==> tables/improv.tex <==
\begin{table*}\centering 
\renewcommand{\arraystretch}{1.1}
\caption{Average Improvement Comparing to Original Models}
\label{improve-table}
\begin{threeparttable}
\begin{tabular}{cccccccc}
\hline
\multicolumn{2}{c}{} & \multicolumn{2}{c}{Epinion} & \multicolumn{2}{c}{MovieLens} & \multicolumn{2}{c}{Gowalla}  \\\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}

\multicolumn{2}{c}{} & Overall $\uparrow$ & \UOFMatric $\downarrow$ & Overall $\uparrow$& \UOFMatric $\downarrow$ & Overall $\uparrow$ & \UOFMatric $\downarrow$\\ \hline

\multirow{4}{*}{NDCG} & S-DRO & -0.0020 (-0.57\%) & 0.0114 (74.96\%) & 0.0015 (0.35\%) & 0.0177 (30.91\%) & -0.0025 (-0.62\%) & 0.0202 (22.21\%)\\

 & UFR & 0.0003 (0.09\%) & 0.0119 (59.55\%) & 0.0067 (1.46\%) & 0.0247 (65.71\%) & -0.0021 (-0.51\%) & 0.0278 (31.69\%) \\

& \M & 0.0264 (7.17\%) & 0.0238 (299.49\%) & 0.0361 (7.99\%) & 0.0552 (499.04\%) & 0.0378 (9.4\%) & 0.0518 (100.04\%) \\ \cline{2-8}

& Improv. & \textbf{8700.00\%} & \textbf{100.00\%} & \textbf{438.81\%} & \textbf{123.48\%} & / & \textbf{86.33\%} \\ \hline

\multirow{4}{*}{F1} & S-DRO & -0.0006 (-0.57\%) & 0.0015 (18.19\%) & 0.0000 (0.00\%) & 0.0025 (25.12\%) & -0.0002 (-0.17\%) & 0.0037 (29.07\%) \\

& UFR & -0.0030 (-2.65\%) & 0.0065 (115.96\%) & -0.0009 (-0.67\%) & 0.0081 (309.9\%) & -0.0034 (-2.95\%) & 0.0115 (303.84\%) \\

& \M & 0.0087 (8.01\%) & 0.0097 (798.21\%) & 0.0090 (6.78\%) & 0.0088 (534.31\%) & 0.0107 (9.29\%) & 0.0124 (394.97\%) \\ \cline{2-8}

& Improv. & / & \textbf{49.23\%} & / & \textbf{8.64\%} & / & \textbf{7.83\%} \\ \hline 

\end{tabular}
\begin{tablenotes}
        \footnotesize
        \item[*] Note that the result is the average improvement of overall performance and the average decrease of \UOFMatric~compared with four backbone models. A higher overall performance means better recommendation performance, while a lower \UOFMatric~value means a fairer model. 
        \item[*] Improvement (Improv.) is calculated based on how much more effect \M~can do to the backbone model compared to the best performance between UFR and S-DRO. Sometimes UFR and S-DRO negatively affect the original model, and we don't show improvement in this situation.
      \end{tablenotes}
    \end{threeparttable}
\end{table*}
